Privacy Leakage over Dependent Attributes in One-Sided Differential Privacy

Providing a provable privacy guarantees while maintaining the utility of data is a challenging task in many real-world applications. Recently, a new framework called One-Sided Differential Privacy (OSDP) was introduced that extends existing differential privacy approaches. OSDP increases the utility of the data by taking advantage of the fact that not all records are sensitive. However, the previous work assumed that all records are statistically independent from each other. Motivated by occupancy data in building management systems, this paper extends the existing one-sided differential privacy framework. In this paper, we quantify the overall privacy leakage when the adversary is given dependency information between the records. In addition, we show how an optimization problem can be constructed that efficiently trades off between the utility and privacy.

==> __latexindent_temp.tex <==
\section{Problem Statement and Motivation}
\label{sec:problem}
OSDP is an attractive solution for many practical applications due to its ease of implementation and provable privacy guarantees it provides. One application we studied is a building management system as part of the TIPPERS project \cite{mehrotra2016tippers}.

Figure \ref{fig:occupancy} shows an example of an occupancy pattern for a space in an office building generated by the Building Analytics App \cite{ghayyur2018iot}. Occupancy level 1 indicates that the particular space was occupied and 0 indicates otherwise. A quick inspection of the plot reveals that one can infer many attributes regarding the occupant of the space. For example, one can infer the starting time of the employee by examining when the occupancy level turns to 1 at the beginning of the day as well as when the employee leaves the office. In addition, one can also infer how many times the employee leaves the space and how long it takes for the employee to come back to the space on average. 

\begin{figure}[h]
    \centering
    \includegraphics[width=3.5in]{Figures/occupancy.eps}
    \caption{Occupancy pattern of an office space generated using Building Analytics App \cite{ghayyur2018iot}. Occupancy level 1 indicates that the space is occupied and level 0 indicates the space is not occupied.}
    \label{fig:occupancy}
\end{figure}

Such attributes can be useful in many building applications including energy as well as space optimization.
For example, a commercial building typically has a default work hours setting (ex: 8:00 am to 5:00 pm) when all lights are turned on. However, a lighting control coupled with occupancy sensors would enable more energy efficient lighting control \cite{thomas2009building}. This could be done by looking at average start time per space, and if the space does not become occupied after the default starting hour on average (ex: 9:00 am), then the lighting control can customize the lighting schedule to either match the average starting time of the space or only turn on the light based on the detected occupancy data.

Such lighting control will require average starting times of spaces occupancy to customize its schedule. However, the lighting control would not require the average occupancy level of spaces during the default work hours.  On the other hand, the average occupancy level (fraction of times when the space is occupied during the work hour) information would be required for other types of applications including space optimization \cite{mahasenan2018building}.

While the occupancy data and the attributes that pertain to the data can enable more efficient operation of buildings, many of these attributes are also potentially sensitive information for the occupants. One potential solution to provide privacy to the occupants while enabling these applications is OSDPRR. Given that different applications require different sets of attributes to perform their respective functionalities, OSDPRR can be implemented per attribute. However, as often is the case, there is no guarantee that the records from different attributes are statistically independent from each other. Moreover, it is also possible that two or more applications are colluding and actively exchanging information obtained from queries. 

\begin{figure}[h]
    \centering
    \includegraphics[width=3.6in]{Figures/framework.eps}
    \caption{Illustration of an use case of occupancy data for building management. The dashed lines indicate queries and responses from multiple applications, and the red solid lines indicate additional information including the dependency information between the attributes as well as the exchanged queries responses between colluding applications. }
    \label{fig:framework}
\end{figure}

This implies that when releasing the data under OSDP, the query response mechanisms needs to take into account additional privacy leakage through statistical dependency as well as potential colluding scenarios. Figure \ref{fig:framework} illustrates an example of occupancy driven building applications where each application will be given the query response as well as additional information from statistical dependency of records and other query responses from exchanging information with other applications. 

In the following Section, we will show how to quantify privacy leakage from such additional information under OSDPRR. 





